Load Estimation in a Two-Priority mMTC Random Access Channel

The use of cellular networks for massive machine-type communications (mMTC) is an appealing solution due to the wide availability of cellular infrastructure. Estimating the number of devices (network load) is vital for efficient allocation of the available resources, especially for managing the random access channel (RACH) of the network. This paper considers a two-priority RACH and proposes two network load estimators: a maximum likelihood (ML) estimator and a reduced complexity (RCML) variant. The estimators are based on a novel model of the random access behavior of the devices coupled with a flexible analytical framework to calculate the involved probabilities. Monte Carlo simulations demonstrate the accuracy of the proposed estimators for different network configurations.

==> Preamble/Nomenclature.tex <==
\nomenclature[P]{\(M\)}{The number of RBs}
\nomenclature[P]{\(n^h\)}{The number of H-UEs}
\nomenclature[P]{\(n^l\)}{The number of L-UEs}
\nomenclature[P]{\(n\)}{The total number of UEs}
\nomenclature[P]{\(N^h\)}{The remaining number of H-UEs}
\nomenclature[P]{\(N^l\)}{The remaining number of L-UEs}
\nomenclature[P]{\(N\)}{The remaining number of UEs}
\nomenclature[P]{\(T\)}{The number of time slots}

\nomenclature[T]{\(\mathbf{p}^h\)}{The probability vector that a H-UE chooses an RB}
\nomenclature[T]{\(\mathbf{p}^l\)}{The probability vector that a H-UE chooses an RB}
\nomenclature[V]{\(p^h_i\)}{The probability that a H-UE chooses RB \(i\)}
\nomenclature[V]{\(p^l_i\)}{The probability that a H-UE chooses RB \(i\)}
\nomenclature[T]{\(\bm{\pi}_t\)}{The access pattern at time slot \(t\)}
\nomenclature[V]{\(z\)}{The intermediate variable used in the derivation of the collision probability}

\nomenclature[E]{\(h\)}{The event that an RB is occupied by a single H-UE}
\nomenclature[E]{\(l\)}{The event that an RB is occupied by a single H-UE}
\nomenclature[E]{\(\phi\)}{The event that an RB is not occupied by any UE}
\nomenclature[E]{\(x\)}{The event that an RB is occupied by two or more UEs}

\nomenclature[E]{\(H_i\)}{The event that a single H-UE occupies RB \(i\)}
\nomenclature[E]{\(L_i\)}{The event that a single H-UE occupies RB \(i\)}
\nomenclature[E]{\(\Phi_i\)}{The event that no UE occupies RB \(i\)}
\nomenclature[E]{\(X_i\)}{The event that two or more UEs occupy RB \(i\)}

\nomenclature[S]{\(\mathcal{H}\)}{The set of RB indices containing only one H-UE}
\nomenclature[S]{\(\mathcal{L}\)}{The set of RB indices containing only one H-UE}
\nomenclature[S]{\(\mathbf{\mathit{\Phi}}\)}{The set of RB indices containing no UE}
\nomenclature[S]{\(\mathcal{X}\)}{The set of RB indices containing two or more UEs}

\nomenclature[V]{\(H_{\bm{\pi}}\)}{The length of \(\mathcal{H}\) of pattern \(\bm{\pi}\)}
\nomenclature[V]{\(L_{\bm{\pi}}\)}{The length of \(\mathcal{L}\) of pattern \(\bm{\pi}\)}
\nomenclature[V]{\(\Phi_{\bm{\pi}}\)}{The length of \(\mathbf{\mathit{\Phi}}\) of pattern \(\bm{\pi}\)}
\nomenclature[V]{\(X_{\bm{\pi}}\)}{The length of \(\mathcal{X}\) of pattern \(\bm{\pi}\)}

% Variables associated with backtracking algorithms
\nomenclature[T]{\(\mathbf{s}\)}{The intermediate sub-vector representing partial solutions during the backtracking process}
\nomenclature[S]{\(\mathcal{N}\)}{The set of outputs from recursive calls of the backtracking algorithm}
\nomenclature[T]{\(\mathbf{k}\)}{The vector representing a feasible allocation of UEs to the RBs in \(\mathcal{X}\)}
\nomenclature[V]{\(\text{UEs}_{\text{max}}\)}{The maximum number of UEs that can be assigned to a single RB while ensuring a collision in the remaining RBs in \(\mathcal{X}\)}

\nomenclature[V]{\(H_{\bm{\pi},p}\)}{The partial number of successful H-UEs of a given access pattern \(\bm{\pi}\)}
\nomenclature[V]{\(L^T_{\bm{\pi},p}\)}{The partial number of successful L-UEs of a given access pattern \(\bm{\pi}\)}
\nomenclature[V]{\(T^T_{\bm{\pi},p}\)}{The partial minimum number of UEs required to ensure that the of the access pattern \(\bm{\pi}\) is feasible}
\nomenclature[V]{\(X^T_{\bm{\pi},p}\)}{The partial number of collisions of a given access pattern \(\bm{\pi}\)}

\nomenclature[S]{\(\mathcal{K}\)}{The set of vectors, each representing a feasible UE allocation to the RBs in \(\mathcal{X}\) (output from \textsc{FindCombinations})}
\nomenclature[S]{\(\mathcal{I}\)}{The set of vectors, each representing a feasible allocation of H-UEs to the RBs in \(\mathcal{X}\) (output from \textsc{FindCombinationsH})}
\nomenclature[S]{\(\mathcal{P}\)}{The set of vectors, each representing a feasible access pattern (output from \textsc{FindPatternCombinations})}

\nomenclature[P]{\(r\)}{The discretization step size}
\nomenclature[S]{\(\mathcal{AS}\)}{The set of vectors, each vector contains two sub-vectors, $\mathbf{p}^h$ and $\mathbf{p}^l$ (output from \textsc{DiscretizeAs} and \textsc{DiscretizeAsCs})}
\nomenclature[T]{\(\mathbf{p}^h_p\)}{{The partial probability vector that a H-UE chooses an RB}}
\nomenclature[T]{\(\mathbf{p}^l_p\)}{{The partial probability vector that a H-UE chooses an RB}}
\nomenclature[S]{\(\mathcal{E}\)}{The set of existing probability vector pairs}
\nomenclature[S]{\(\mathcal{CS}\)}{The set of circular shifts of the current probability vector pair}
\nomenclature[T]{\(\mathbf{cs}\)}{The elements in $\mathcal{CS}$, which are probability vector pairs}

\nomenclature[P]{\(\gamma\)}{The H-UE RACH throughput threshold}
\nomenclature[P]{\(runs\)}{The number of runs for the MAB alg.}
\nomenclature[P]{\(B_s\)}{The batch size}
\nomenclature[V]{\(B_e\)}{The 'elite' batch size}
\nomenclature[P]{\(\rho\)}{The portion of the batch size that is used as the 'elite' batch size}
\nomenclature[P]{\(\alpha\)}{The learning rate}


\nomenclature[T]{\(\mathbf{p}^{\mathcal{AS}}\)}{The probability vector for selecting an action in the AS}
\nomenclature[T]{\(\mathbf{Q}\)}{The vector of length $|\mathcal{AS}|$, representing the action-value function}
\nomenclature[T]{\(\mathbf{v}\)}{The vector of length $|\mathcal{AS}|$, representing the number of times each action is selected}
\nomenclature[V]{\(N_a\)}{The number of actions}

==> Preamble/code_listings.tex <==
\usepackage{listings} % for code listings
% General Setting of listings
\lstset{
    aboveskip=1em,
    breaklines=true,
    abovecaptionskip=-6pt,
    captionpos=b,
    escapeinside={\%*}{*)},
    frame=single,
    % numbers=left,
    % numbersep=15pt,
    % numberstyle=\tiny,
}
% 0. Basic Color Theme
\lstdefinestyle{colored}{ %
    basicstyle=\ttfamily,
    backgroundcolor=\color{white},
    commentstyle=\color{green}\itshape,
    keywordstyle=\color{blue}\bfseries\itshape,
    stringstyle=\color{red},
}
% 1. General Python Keywords List
\lstdefinelanguage{PythonPlus}[]{Python}{
    morekeywords=[1]{as, assert, nonlocal, with, yield, self, True, False, None}, % Python builtin
    morekeywords=[2]{__init__, __add__, __mul__, __div__, __sub__, __call__, __getitem__, __setitem__, __eq__, __ne__, __nonzero__, __rmul__, __radd__, __repr__, __str__, __get__, __truediv__, __pow__, __name__, __future__, __all__}, % magic methods
    morekeywords=[3]{object, type, isinstance, copy, deep copy, zip, enumerate, reversed, list, set, len, dict, tuple, range, append, executive, real, imag, reduce, str, repr}, % common functions
    morekeywords=[4]{Exception, NameError, IndexError, SyntaxError, TypeError, ValueError, OverflowError, ZeroDivisionError}, % errors
    morekeywords=[5]{, ode, solve, sqrt, exp, sin, cos, arctan,arctan2, arccos, pi, array, norm, solve, dot, arange, isscalar, max, sum, flatten, shape, reshape, find, any, all, abs, plot, linspace, legend, quad, polyval, polyfill, stack, concatenate, stack, column_stack, empty, zeros, ones, rand, Vander, grid, color,eig, eggs, rivals, svd, QR, tan,det, logspace, roll, min, mean, cumsum, pump rod, diff, vectorize, lists, cla, eye, xlabel, ylabel, show, figure, squeeze}, % numpy / math
    %morekeywords=[6]{tqdm, trange}, % tqdm
}
% 2. New Language based on Python
\lstdefinelanguage{PyBrIM}[]{PythonPlus}{
    emph={d, E, a, Fc28, Fy, Fu, D, des, supplier, Material, Rectangle, PyElmt},
}
% 3. Extended theme
\lstdefinestyle{colorEX}{
    basicstyle=\ttfamily,
    backgroundcolor=\color{white},
    commentstyle=\color{darkgreen}\slshape,
    keywordstyle=\color{blue}\bfseries\itshape,
    keywordstyle=[2]\color{blue}\bfseries,
    keywordstyle=[3]\color{grass},
    keywordstyle=[4]\color{red},
    keywordstyle=[5]\color{orange},
    stringstyle=\color{darkred},
    emphstyle=\color{pink}\underbar,
}
\lstset{style=colorEX}

